Vision Transformer Pruning Via Matrix Decomposition

This is a further development of Vision Transformer Pruning via matrix decomposition. The purpose of the Vision Transformer Pruning is to prune the dimension of the linear projection of the dataset by learning their associated importance score in order to reduce the storage, run-time memory, and computational demands. In this paper we further reduce dimension and complexity of the linear projection by implementing and comparing several matrix decomposition methods while preserving the generated important features. We end up selected the Singular Value Decomposition as the method to achieve our goal by comparing the original accuracy scores in the original Github repository and the accuracy scores of using those matrix decomposition methods, including Singular Value Decomposition, four versions of QR Decomposition, and LU factorization.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

==> preamble.tex <==
\usepackage{xspace}

%Here we define a marco: The \xspace ensures correct spacing, i.e. insert space before next word, but not before period or comma.
\newcommand{\paxos}{\textsc{Paxos}\xspace}

%These packages are needed for the plot in Figure 1. 
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}



==> tex/background.tex <==
Give a short, self-contained summary of necessary background
information. 

For our example if your project is a new \paxos implementation, the background
would be a brief introduction to the consensus problem, the \paxos algorithm,
the system model used by the \paxos algorithm
and common optimizations and relevant variations of that algorithm.

The goal of the background section is to make the paper 
self-contained for an audience as large as possible. As in every
section you start with a very brief overview of the section.
For our example that would be: In this section, we introduce the consensus problem,
the \paxos algorithm and common optimizations of that algorithm.

If you copy a definition from a text book or some other source, you must cite that source. 
See Example~\ref{def:consensus} below. 


==> tex/citations.tex <==
\begin{comment}


It is important that you correctly refer to sources. 

\begin{itemize}
\item If you describe background, according to some textbook, cite that textbook. \emph{See Example~\ref{def:consensus} below.}
\item If you make a claim about trends in industry or research, add citations to validate the claim. \emph{See Example~\ref{ex:trend} below.}
\item \textbf{Do not copy paste text from any source into your report without citation. It will be considered plagiarism.}
\item Always use the tilde character between the text and the cite command, e.g.:\begin{verbatim}
DBLP~\cite{dplg}
\end{verbatim}
The tilde inserts a space, but prevents line break between the text and citation.
\item For correct citations we recommend that you export bibtex entries from DBLP~\cite{dplg}. 
%@Hein: ACM produces crappy doi-urls for non ACM publications. I do believe that there are few papers that are part of the ACM-DL and not in DBLP.
But make sure to update the bibtex entries to adhere to the following rules.
\end{itemize}

Here are some rules to be followed for your bibliography:

\begin{itemize}
\item Make sure titles are correctly capitalized.

%You can export all nsdi citations from DBLP, accordingly this should not be a problem.
% \item Make sure abbreviations are consistent (e.g., is NSDI spelled out or
% not?) - using the @abbrev function in latex helps here.

\item Make sure there is enough info for a reader to find the document: authors
plus title isn't enough.

\item Don't blindly copy and paste ACM bibtex entries without fixing them:

- they list "New York, NY" as the address field, which means that all ACM
conferences look like they took place there; just delete this, or - better

- replace it with where the conference took place, which is much more
helpful to the reader than the publisher's address

- they have a truly weird idea about how to capitalize conference names;
just correct this (consistently)

* IEEE is equally bad, and uses a partially-inverted form of conference
names.

* Please actually review the bibliography before submitting your paper!
\end{itemize}

%@Leander: Move this to the Latex part:

And while you are at it, please:

\begin{itemize}
\item Add include{mathpmtc} in the main LaTeX file, so you don't have
math stuff in a different font than the main text. 
%We could simply add this to the template if not already done.

\item Always use the tilde character between the number and unit, e.g. 100~Mbps or 53~ms. 
The tilde inserts a space, but prevents line break between the number and unit.

\item Never put SI units in italics. 

\item Do differentiate between bits (b) and bytes (B), and between powers of 10~(MB) and 2~(MiB).

\item Avoid things like: "We refer the reader to [42]." That is, don't use citations as nouns.
\end{itemize}


\begin{example}
\label{def:consensus}
Consensus is a distributed programming abstraction that fulfills the following properties~\cite{aTextbook}:
\begin{description}
\item[Termination]
\item[Validity]
\item[Integrity]
\item[Agreement]
\end{description}
\end{example}

\noindent
\begin{example}
\label{ex:trend} Consensus systems build a fundamental part of todays cloud-computing infrastructure~\cite{spanner,chubby,zookeeper,zookeeperWeb}.
\end{example}
\end{comment}


==> tex/latex.tex <==
This section contains some instructions and examples for using \LaTeX.

\subsection{You can add subsections}
You can use numbered subsections to structure your sections or $\backslash\texttt{paragraph}$ to separate paragraphs with a heading using only a few words, as used in Section~\ref{sec:introduction}.


\begin{enumerate}
	\item\label{item:1} This is an item in an enumeration.
    \begin{itemize}
    	\item This is an item of a unnumbered list. In this case, the lists are nested within each other.
    \end{itemize}
    \item\label{item:2} The second point in the enumerated list.
\end{enumerate}
%
I can refer to the element of the enumeration above as Point~\ref{item:1}.
If you refer to numbered items,~e.g. items from a list or figures or sections, always capitalize the name. 
For example, this is Section~\ref{sec:latex}.

\subsection{Figures}
You can include figures. You can include files, as done in Figure~\ref{fig:example}. 
Avoid including jpeg, gif or bmp files since these do not scale nicely. Again Figure~\ref{fig:example} is an example for that.

\begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{fig/RegisterOperations}
    \caption{Figure taken from~\cite{lecture}}
    \label{fig:example}
\end{figure}

You can create graphs from your experiment-data using \texttt{pgfplots}.
See the example in \texttt{tex/evaluation.tex} and documentation \url{http://pgfplots.sourceforge.net/pgfplots.pdf}.

\subsection{Other tips}
\begin{itemize}

\item Always use the tilde character between the number and unit, e.g. 100~Mbps or 53~ms. The tilde inserts a space, but prevents line break between the number and unit.

\item Never put SI units in italics. 

\item Do differentiate between bits (b) and bytes (B), and between powers of 10~(MB) and 2~(MiB).

\item Avoid things like: "We refer the reader to [42]." That is, don't use citations as nouns.
\end{itemize}

For further instructions on how to add \textbf{Tables, Algorithms, Theorems see acmguide.pdf}.

